Comparison of Polar Decoders with Existing Low-Density Parity-Check and Turbo Decoders

Polar codes are a recently proposed family of provably capacity-achieving error-correction codes that received a lot of attention. While their theoretical properties render them interesting, their practicality compared to other types of codes has not been thoroughly studied. Towards this end, in this paper, we perform a comparison of polar decoders against LDPC and Turbo decoders that are used in existing communications standards. More specifically, we compare both the error-correction performance and the hardware efficiency of the corresponding hardware implementations. This comparison enables us to identify applications where polar codes are superior to existing error-correction coding solutions as well as to determine the most promising research direction in terms of the hardware implementation of polar decoders.

==> tables/ADHardwareTable.tex <==
\begin{tabular}{rrrrrrrrrr}
\hline
Work 	& N & Tech. & Area 		& Freq. & Schedule & Iter. & T/P 		& Voltage & Power \\
			&		&	(nm)	& (mm$^2$)& (MHz)	&					 &       & (Mb/s)	& (V) 		& (mw) \\
\hline
Shrirani-Mehr \emph{et al.} \cite{Shirani-mehr2011} & $672$ & $65$ & $0.72$ & $235$ & Layered& $5$ & $7900$ & n/a & n/a \\
Weiner \emph{et al.} \cite{Weiner2011} & $672$ & $65$ & $1.30$ & $150$ & Flooding& $15$ & $3080$ & $0.8$ & $84$ \\
Yen \emph{et al.} \cite{Yen2012} & $672$ & $65$ & $1.56$ & $197$ & Layered& $5$ & $5790$ & $1.0$ & $361$ \\
Ajaz \emph{et al.} \cite{Ajaz2013} & $672$ & $65$ & $1.10$ & $215$ & Layered& $6$ & $6000$ & $1.1$ & $210$ \\
Balatsoukas-Stimming \emph{et al.} \cite{Balatsoukas2013} & $672$ & $40$ & $0.18$ & $850$ & Layered& $5$ & $3120$ & n/a & n/a \\
Li \emph{et al.} \cite{Li2013a} & $672$ & $40$ & $0.16$ & $500$ & Layered& $5$ & $5600$ & $0.9$ & $99$ \\
Li \emph{et al.} \cite{Li2013b} & $672$ & $40$ & $0.22$ & $500$ & Layered& $5$ & $5300$ & $0.9$ & $136$ \\
Park \emph{et al.} \cite{Park2014b} & $672$ & $65$ & $1.60$ & $540$ & Flooding& $10$ & $9000$ & $1.1$ & $783$ \\
Ajaz \emph{et al.} \cite{Ajaz2014} & $672$ & $65$ & $0.57$ & $400$ & Layered& $7$ & $9250$ & $1.1$ & $273$ \\
Weiner \emph{et al.} \cite{Weiner2014} & $672$ & $28$ & $0.63$ & $65$ & Flooding& $15$ & $6000$ & $0.7$ & $38$ \\
Li \emph{et al.} \cite{Li2015} & $672$ & $28$ & $0.13$ & $400$ & Layered& $3$ & $7070$ & $0.8$ & $54$ \\
Li \emph{et al.} \cite{Li2015b} & $672$ & $28$ & $0.78$ & $470$ & Layered& $5$ & $18400$ & $0.9$ & $166$ \\
\hline
\end{tabular}


==> tables/BPHardwareTable.tex <==
\begin{tabular}{rrrrrrrrrr}
\hline
Work 	& Main Contribution & N & Tech. & Area 		& Freq. & Max.  & Max. T/P	& Sust. T/P & Power \\
			&										&		&	(nm)	& (mm$^2$)& (MHz)	&	Iter.	& (Mb/s)		& (Mb/s)		& (mW) \\
\hline
Park \emph{et al.} \cite{Park2014} & Unidirectional schedule. & $1024$ & $65$ & $1.48$ & $300$ & $15$ & $4676$ & $2048$ & $478$ \\
Yuan \emph{et al.} \cite{Yuan2014} & Early termination. & $1024$ & $45$ & $1.04$ & $500$ & $40$ & $4500$ & $2588$ & $990$ \\
Abbas \emph{et al.} \cite{Abbas2015} & Sub-graph freezing. & $1024$ & $45$ & $0.75$ & $197$ & $15$ & $1683$ & $1683$ & n/a \\
Lin \emph{et al.} \cite{Sun2016} & Adaptive quantization. & $1024$ & $65$ & $1.40$ & $769$ & $5$ & $7870$ & $7870$ & $442$ \\
\hline
\end{tabular}


==> tables/DVBS2HardwareTable.tex <==
\begin{tabular}{rrrrrrrrr}
\hline
Work & N & Tech. (nm) & Area (mm$^2$) & Freq. (MHz) & Iter. & T/P (Mb/s) & Voltage (V) & Power (mW) \\
\hline
Kienle \emph{et al.} \cite{Kienle2005} & $64800$ & $130$ & $22.74$ & $270$ & $30$ & $0$ & n/a & n/a \\
Dielissen \emph{et al.} \cite{Dielissen2006} & $64800$ & $90$ & $4.10$ & n/a & $30$ & $0$ & n/a & n/a \\
Urard \emph{et al.} \cite{Urard2005} & $64800$ & $90$ & $6.07$ & $300$ & $30$ & $0$ & $1.0$ & $700$ \\
Urard \emph{et al.} \cite{Urard2008} & $64800$ & $65$ & $15.80$ & $174$ & $30$ & $0$ & $1.2$ & $476$ \\
M{\"u}ller \emph{et al.} \cite{Muller2009} & $64800$ & $90$ & $13.10$ & $270$ & $50$ & $0$ & $1.0$ & $853$ \\
M{\"u}ller \emph{et al.} \cite{Zhang2009} & $64800$ & $90$ & $9.60$ & $320$ & $30$ & $0$ & n/a & n/a \\
\hline
\end{tabular}


==> tables/GE10HardwareTable.tex <==
\begin{tabular}{rrrrrrrrrr}
\hline
Work 	& N & Tech. & Area		& Freq. & Schedule & Iter. 	& T/P  	& Voltage & Power \\
			&		&	(nm)	& (mm$^2$)& (MHz)	&					 & 				& (Mb/s)& (V)			& (mW) \\
\hline
Cevrero \emph{et al.} \cite{Cevrero2010} & $2048$ & $90$ & $5.35$ & $137$ & Layered& $4$ & $11690$ & $1.2$ & $1559$ \\
Zhang \emph{et al.} \cite{Zhang2010} & $2048$ & $65$ & $5.35$ & $100$ & Flooding& $8$ & $6670$ & $0.7$ & $144$ \\
Zhang \emph{et al.} \cite{Zhang2010} & $2048$ & $65$ & $5.35$ & $700$ & Flooding& $8$ & $47700$ & $1.2$ & $2800$ \\
Bao \emph{et al.} \cite{Bao2012} & $2048$ & $130$ & $18.40$ & $278$ & Layered& $5$ & $9480$ & $1.2$ & $774$ \\
\hline
\end{tabular}


==> tables/LTEHardwareTable.tex <==
\begin{tabular}{rrrrrrrrr}
\hline
Work 	& K & Tech. & Area 		& Freq. & Iter. 	& T/P 	& Voltage & Power \\
			&		&	(nm)	& (mm$^2$)& (MHz)	&					& (Mb/s)& (V)			& (mW) \\
\hline
Studer \emph{et al.} \cite{Studer2011} & $6144$ & $130$ & $3.57$ & n/a & $6$ & $391$ & $1.2$ & $789$ \\
Ilnseher \emph{et al.} \cite{Ilnseher2012} & $6144$ & $65$ & $7.70$ & $450$ & $6$ & $2150$ & $1.1$ & n/a \\
Chen \emph{et al.} \cite{Chen2013b} & $6144$ & $65$ & $1.39$ & $512$ & $6$ & $692$ & $1.2$ & $635$ \\
Lin \emph{et al.} \cite{Lin2013} & $6144$ & $40$ & $1.27$ & $252$ & $6$ & $535$ & $0.9$ & $218$ \\
Belfanti \emph{et al.} \cite{Belfanti2013} & $6144$ & $65$ & $2.49$ & $410$ & $6$ & $1013$ & $1.2$ & $966$ \\
Shrestha \emph{et al.} \cite{Shrestha2014} & $6144$ & $45$ & $2.43$ & $600$ & $6$ & $1067$ & $0.8$ & $870$ \\
Wang \emph{et al.} \cite{Wang2014} & $6144$ & $90$ & $6.10$ & $625$ & $8$ & $438$ & $1.0$ & $272$ \\
Wang \emph{et al.} \cite{Wang2014} & $6144$ & $90$ & $19.75$ & $625$ & $8$ & $2274$ & $1.0$ & $1450$ \\
\hline
\end{tabular}


==> tables/NHardwareTable.tex <==
\begin{tabular}{rrrrrrrrrr}
\hline
Work 	& N & Tech.	& Area		& Freq. & Schedule & Iter.  & T/P		& Voltage	& Power \\
			&		&	(nm)	& (mm$^2$)& (MHz)	&					 & 				& (Mb/s)& (V)			& (mW) \\
\hline
Gunnam \emph{et al.} \cite{Gunnam2007} & $1944$ & $130$ & $1.85$ & $500$ & Layered& $15$ & $1618$ & n/a & $238$ \\
Rovini \emph{et al.} \cite{Rovini2007} & $1944$ & $65$ & $0.48$ & $240$ & Layered& $12$ & $196$ & $1.2$ & $168$ \\
Rovini \emph{et al.} \cite{Rovini2007b} & $1944$ & $65$ & $0.74$ & $240$ & Layered& $12$ & $178$ & $1.2$ & $234$ \\
Studer \emph{et al.} \cite{Studer2008} & $1944$ & $180$ & $3.39$ & $208$ & Layered& $5$ & $780$ & n/a & $2886$ \\
Sun \emph{et al.} \cite{Sun2009} & $2304$ & $65$ & $1.20$ & $400$ & Layered& $10$ & $415$ & $0.9$ & $180$ \\
Jin \emph{et al.} \cite{Jin2010} & $1944$ & $180$ & $2.67$ & $250$ & Layered& $10$ & $503$ & $1.8$ & $463$ \\
Roth \emph{et al.} \cite{Roth2010} & $1944$ & $90$ & $1.77$ & $346$ & Layered& $10$ & $679$ & $1.0$ & $107$ \\
Sun \emph{et al.} \cite{Sun2011} & $1944$ & $45$ & $0.81$ & $815$ & Layered& $15$ & $3000$ & n/a & n/a \\
Meinerzhagen \emph{et al.} \cite{Meinerzhagen2015} & $1944$ & $90$ & $1.00$ & $307$ & Layered& $10$ & $600$ & $1.0$ & $88$ \\
\hline
\end{tabular}


==> tables/SCHardwareTable.tex <==
\begin{tabular}{rrrrrrrr}
\hline
Work 	& Main Contribution & N & Tech. & Area		& Freq. & T/P		& Power \\
			&										&		&	(nm)	& (mm$^2$)& (MHz)	&	(Mb/s)& (mW) \\
\hline
Leroux \emph{et al.} \cite{Leroux2012} & Linear memory requirement. & $1024$ & $65$ & $0.36$ & $500$ & $239$ & n/a \\
Mishra \emph{et al.} \cite{Mishra2012} & First ASIC, two-bit decoding. & $1024$ & $180$ & $1.71$ & $150$ & $98$ & $67$ \\
Leroux \emph{et al.} \cite{Leroux2013} & Semi-parallel architecture. & $1024$ & $65$ & $0.31$ & $500$ & $246$ & n/a \\
Fan \emph{et al.} \cite{Fan2014} & Efficient partial sum computation. & $1024$ & $65$ & $0.07$ & $1010$ & $497$ & n/a \\
Yuan \emph{et al.} \cite{Yuan2014b} & Two-bit decoding with precomputation. & $1024$ & $45$ & $0.64$ & $750$ & $1000$ & n/a \\
Lin \emph{et al.} \cite{Lin2015a} & SCAN decoder. & $1024$ & $90$ & $0.97$ & $571$ & $958$ & n/a \\
Che \emph{et al.} \cite{Che2015} & Implementation of fast-SSC decoding. & $1024$ & $45$ & $0.28$ & $1040$ & $4004$ & n/a \\
Dizdar \emph{et al.} \cite{Dizdar2016} & Single-cycle implementation. & $1024$ & $90$ & $3.21$ & $2$ & $2560$ & $191$ \\
Giard \emph{et al.} \cite{Giard2016} & Fast-SSC decoding for low-rate codes. & $1024$ & $65$ & $0.69$ & $600$ & $3720$ & $215$ \\
Giard \emph{et al.} \cite{Giard2016b} & Unrolled decoder implementation. & $1024$ & $65$ & $1.44$ & $650$ & $25600$ & $546$ \\
Lin \emph{et al.} \cite{Lin2016} & Fast-SSC SCAN decoder. & $1024$ & $90$ & $1.01$ & $471$ & $1435$ & n/a \\
\hline
\end{tabular}


==> tables/SCLHardwareTableL2.tex <==
\begin{tabular}{rrrrrrr}
\hline
Work 	& Main Contribution & N & Tech. & Area 		& Freq.	& T/P \\
			&										&		&	(nm)	& (mm$^2$)& (MHz)	&	(Mb/s)\\
\hline
Balatsoukas-Stimming \emph{et al.} \cite{Balatsoukas2014b} & First architecture, efficient path copying. & $1024$ & $90$ & $1.38$ & $794$ & $314$ \\
Lin \emph{et al.} \cite{Lin2014} & First CRC-aided decoder. & $1024$ & $90$ & $1.77$ & $714$ & $285$ \\
Balatsoukas-Stimming \emph{et al.} \cite{Balatsoukas2015} & LLR-based reformulation and implementation. & $1024$ & $90$ & $0.88$ & $847$ & $335$ \\
Fan \emph{et al.} \cite{Fan2015} & Low-complexity path metric sorting. & $1024$ & $90$ & n/a & n/a & n/a \\
Hashemi \emph{et al.} \cite{Hashemi2016} & Reduced memory requirements. & $2048$ & $90$ & $0.91$ & $500$ & $164$ \\
Lin \emph{et al.} \cite{Lin2015b} & Efficient memory structure and metric sorting. & $1024$ & $90$ & $0.55$ & $500$ & $181$ \\
Lin \emph{et al.} \cite{Lin2015c} & Fast-SSC SCL decoding with approximations. & $1024$ & $90$ & $1.98$ & $423$ & $1332$ \\
Xiong \emph{et al.} \cite{Xiong2015} & Partial ML decoding, flexible architecture. & $1024$ & $90$ & n/a & n/a & n/a \\
Yuan \emph{et al.} \cite{Yuan2015} & Multi-bit decision LL-based SCL decoding. & $1024$ & $65$ & $1.06$ & $500$ & $501$ \\
Xiong \emph{et al.} \cite{Xiong2016} & Symbol-based SCL decoding. & $1024$ & $90$ & n/a & n/a & n/a \\
Yuan \emph{et al.} \cite{Yuan2016} & Multi-bit decision LLR-based SCL decoding. & $1024$ & $65$ & n/a & n/a & n/a \\
\hline
\end{tabular}


==> tables/SCLHardwareTableL4.tex <==
\begin{tabular}{rrrrrrr}
\hline
Work 	& Main Contribution & N & Tech. & Area  	& Freq. & T/P \\
			&										&		&	(nm)	& (mm$^2$)& (MHz)	&	(Mb/s)\\
\hline
Balatsoukas-Stimming \emph{et al.} \cite{Balatsoukas2014b} & First architecture, efficient path copying. & $1024$ & $90$ & $2.62$ & $730$ & $288$ \\
Lin \emph{et al.} \cite{Lin2014} & First CRC-aided decoder. & $1024$ & $90$ & $3.02$ & $657$ & $216$ \\
Balatsoukas-Stimming \emph{et al.} \cite{Balatsoukas2015} & LLR-based implementation. & $1024$ & $90$ & $1.78$ & $794$ & $307$ \\
Fan \emph{et al.} \cite{Fan2015} & Low-complexity path metric sorting. & $1024$ & $90$ & n/a & n/a & n/a \\
Hashemi \emph{et al.} \cite{Hashemi2016} & Reduced memory requirements. & $2048$ & $90$ & $1.36$ & $500$ & $164$ \\
Lin \emph{et al.} \cite{Lin2015b} & Efficient memory and metric sorting. & $1024$ & $90$ & $1.13$ & $476$ & $173$ \\
Lin \emph{et al.} \cite{Lin2015c} & Fast-SSC decoding with approximations. & $1024$ & $90$ & $3.83$ & $403$ & $1140$ \\
Xiong \emph{et al.} \cite{Xiong2015} & Partial ML decoding, flexibility. & $1024$ & $90$ & $1.89$ & $409$ & $1094$ \\
Yuan \emph{et al.} \cite{Yuan2015} & Multi-bit decision LL-based decoding. & $1024$ & $65$ & $2.14$ & $400$ & $401$ \\
Xiong \emph{et al.} \cite{Xiong2016} & Symbol-based SCL decoding. & $1024$ & $90$ & $1.21$ & $500$ & $313$ \\
Yuan \emph{et al.} \cite{Yuan2016} & Multi-bit decision LLR-based decoding. & $1024$ & $65$ & $1.18$ & $360$ & $675$ \\
\hline
\end{tabular}

